Design Method of a Kangaroo Robot with High Power Legs and an Articulated Soft Tail

In this paper, we focus on the kangaroo, which has powerful legs capable of jumping and a soft and strong tail. To incorporate these unique structure into a robot for utilization, we propose a design method that takes into account both the feasibility as a robot and the kangaroo-mimetic structure. Based on the kangaroo's musculoskeletal structure, we determine the structure of the robot that enables it to jump by analyzing the muscle arrangement and prior verification in simulation. Also, to realize a tail capable of body support, we use an articulated, elastic structure as a tail. In order to achieve both softness and high power output, the robot is driven by a direct-drive, high-power wire-winding mechanism, and weight of legs and the tail is reduced by placing motors in the torso. The developed kangaroo robot can jump with its hind legs, moving its tail, and supporting its body using its hind legs and tail.

==> preamble.tex <==
\RequirePackage[l2tabu, orthodox]{nag} % 古いコマンドやパッケージの利用を警告する
\usepackage[all, warning]{onlyamsmath} % amsmath が提供しない数式環境を使用した場合に警告
% for not arxiv
% \usepackage[dvipdfmx]{color}
% \usepackage[dvipdfmx,bookmarks=true,bookmarksnumbered=true,bookmarkstype=toc,%
%      colorlinks=true,%
%      linkcolor=black, %%追加20090108
%      citecolor=black, %%追加20090108
%      urlcolor=black, %%追加20090108
%      bookmarksopen=true,%しおりツリーをデフォルトで開く
% %     backref=page,%citeにどこで使っているか出るようになる
%      pdftitle=\PDFTITLE,%
%      pdfsubject=\PDFSUBJECT,%
%      pdfauthor=\PDFAUTHOR,%
%      pdfkeywords=\PDFKEYWORDS]{hyperref}
% %% \usepackage[dvipdfmx]{graphicx}
% \usepackage[dvips]{graphicx}
% \usepackage[dvipdfmx]{}

% for arxiv
\usepackage{hyperref}
\usepackage{color}
\usepackage{graphicx}

% \usepackage{jtygm}
\usepackage{url} % \url のために必要
%% \url{http://nile.ulis.ac.jp/~yuka/}
\usepackage{txfonts,mathptmx}

%%%% カスタマイズしたい場合は以下に書く

\newcommand{\TODO}[1]{\fbox{{\textbf TODO:}#1}}
\usepackage{layout}
\usepackage{wrapfig}

% \usepackage{pxjahyper}
% hypcap: figref, tabrefしたときにジャンプ先がキャプション部ではなく図の上になる
\usepackage[figure,figure*,table,table*]{hypcap}
% \usepackage{eclbkbox}
%% \usepackage[dvipdfmx]{graphicx}
% \usepackage[dvipdfmx]{}
\usepackage{url} % \url のために必要
%% \url{http://nile.ulis.ac.jp/~yuka/}
%\usepackage{html} % latex2html で 利用
\usepackage{algorithm}
\usepackage{algcompatible}
\usepackage{algpseudocode}
\usepackage{amsmath}
\algblockdefx{FORP}{ENDFORP}[1]%
  {\textbf{for}#1 \textbf{do in parallel}}%
  {\textbf{end for}}
\algnewcommand{\algorithmicand}{\textbf{ and }}
\algnewcommand{\algorithmicor}{\textbf{ or }}
\algnewcommand{\OR}{\algorithmicor}
\algnewcommand{\AND}{\algorithmicand}
% \usepackage[subrefformat=parens]{subcaption}
% \captionsetup{compatibility=false} % http://www.yamamo10.jp/yamamoto/comp/latex/make_doc/insert_fig/
% \captionsetup[sub]{skip=4pt}

%% \newcommand{\tabref}[1]{{表~\ref{#1}}~}
%% \newcommand{\figref}[1]{{図~\ref{#1}}~}
%% \newcommand{\equref}[1]{{式(\ref{#1})}~}
\newcommand{\secref}[1]{Section \ref{#1}}
\newcommand{\subsecref}[1]{Subsection \ref{#1}}
\newcommand{\tabref}[1]{{Table \ref{#1}}}
\newcommand{\figref}[1]{{Fig. \ref{#1}}}
%% \newcommand{\figref}[1]{\figurename\ref{fig:#1}}
\newcommand{\equref}[1]{{Eq. \ref{#1}}}
\newcommand{\algoref}[1]{{Alg. \ref{#1}}}
\newcommand{\enumref}[1]{{\ref{#1}}}
%% \renewcommand{\figurename}{Fig.}
%% \renewcommand{\tablename}{Table }

\newcommand{\switchlanguage}[2]{%
  \ifx\paperlanguage\empty%
  #1%
  \else%
  #2%
  \fi%
}

